Multimodal RewardBench 2: Evaluating Omni Reward Models for Interleaved Text and Image

Reward models (RMs) are essential for training large language models (LLMs), but remain underexplored for omni models that handle interleaved image and text sequences. We introduce Multimodal RewardBench 2 (MMRB2), the first comprehensive benchmark for reward models on multimodal understanding and (interleaved) generation. MMRB2 spans four tasks: text-to-image, image editing, interleaved generation, and multimodal reasoning ("thinking-with-images"), providing 1,000 expert-annotated preference pairs per task from 23 models and agents across 21 source tasks. MMRB2 is designed with: (1) practical but challenging prompts; (2) responses from state-of-the-art models and agents; and (3) preference pairs with strong human-expert consensus, curated via an ensemble filtering strategy. Using MMRB2, we study existing judges for each subtask, including multimodal LLM-as-a-judge and models trained with human preferences. The latest Gemini 3 Pro attains 75-80% accuracy. GPT-5 and Gemini 2.5 Pro reach 66-75% accuracy, compared to >90% for humans, yet surpass the widely used GPT-4o (59%). The best performing open-source model Qwen3-VL-32B achieves similar accuracies as Gemini 2.5 Flash (64%). We also show that MMRB2 performance strongly correlates with downstream task success using Best-of-N sampling and conduct an in-depth analysis that shows key areas to improve the reward models going forward.

==> tables/mllm_results.tex <==

\begin{table*}[h]
\centering
% Left (60%)
\begin{minipage}{0.56\textwidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}

\toprule[1.2pt]

Judge & 
\begin{tabular}[c]{@{}c@{}} Text to\\ Image\end{tabular} & 
\begin{tabular}[c]{@{}c@{}} Image\\ Editing\end{tabular} & 
\begin{tabular}[c]{@{}c@{}} Interleaved\\ 
Generation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Multimodal\\ Reasoning\end{tabular} \\ 

\midrule[1.2pt]
% Random & 50.0 & 50.0 & 50.0 & 50.0 \\
% Human-to-human & 95.3 & 96.3 & 95.2 & - \\
% \midrule
\multicolumn{5}{c}{Open-source multimodal LLMs} \\

\midrule


Gemma 3 4B~\citep{gemma}           & 51.7   & 51.0   & 51.3   &  48.8\\
Gemma 3 12B~\citep{gemma}          & 56.0   & 58.0   & 58.0   &  49.3\\
Gemma 3 27B~\citep{gemma}          & 58.3   & 60.2   & 61.1   &  49.4\\
% Llama 4 Scout        & 56.7   & 61.1   & 54.4   &  \\
Qwen2.5-VL-7B~\citep{qwen25vl}          & 50.4   & 57.1   & 48.4   &  47.5\\
Qwen2.5-VL-72B~\citep{qwen25vl}         & 59.1   & 64.6   & 62.3   &  50.0\\
Qwen3-VL-8B~\citep{qwen3vl}          & 59.4   & 61.7   & 61.5   &  54.6\\
Qwen3-VL-32B~\citep{qwen3vl}         & 64.1   & 67.3   & 70.5   &  56.6\\
Qwen3-VL-30BA3B~\citep{qwen3vl}      & 60.0   & 59.5   & 57.3   &  57.3\\
Qwen3-VL-235BA22B~\citep{qwen3vl}    & 62.0   & 64.8   & 69.0   &  55.9\\

\midrule

\multicolumn{5}{c}{API-based Models}\\

\midrule
GPT-4o~\citep{gpt4o}               & 60.3   & 65.0   & 61.5   & 51.9 \\
GPT-4.1~\citep{gpt41}              & 65.8   & 68.2   & 67.0   &  53.0\\
GPT-5~\citep{gpt5}                & \underline{70.5} & \underline{73.8} & 74.4   &  \underline{70.2}\\
Gemini 2.5 Flash~\citep{gemini}     & 63.1   & 66.5   & 69.4   & 57.5 \\
Gemini 2.5 Pro~\citep{gemini}       & \underline{70.5} & 71.3   & \underline{75.1} & 66.6 \\
Gemini 3 Pro~\citep{gemini3pro} & \textbf{74.4} & \textbf{74.9} & \textbf{76.4} & \textbf{79.5} \\

\bottomrule[1.2pt]
\end{tabular}
}
\caption{MLLM-as-a-judge accuracies on MMRB2. The best numbers are \textbf{bolded} and the second best are \underline{underlined}. GPT-5 and Gemini 2.5 Pro are the best across all tasks. Qwen3-VL-32B is the best open-source model.}\label{tab:mllm_results_main}
\end{minipage}
\hfill
% Right (40%)
\begin{minipage}{0.39\textwidth}
\centering
\resizebox{\linewidth}{!}{%

\begin{tabular}{lccc}
\toprule[1.2pt]
Judge & 
\begin{tabular}[c]{@{}c@{}}Text to\\Image\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}Image\\Editing*\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}Multimodal\\Reasoning*\end{tabular} \\
\midrule[1.2pt]
\multicolumn{4}{c}{MLLM-as-a-judge}\\
\midrule
Qwen3-VL-32B~\citep{qwen3vl} & 64.1 & 66.4 & 69.9 \\
GPT-5~\citep{gpt5}       & 70.5 & 74.3 & 83.8 \\
\midrule
\multicolumn{4}{c}{CLIP-based evaluators} \\
\midrule
CLIPScore~\citep{hessel2021clipscore}   & 51.0 & - & - \\
ImageReward~\citep{xu2023imagereward}    & 54.0 & - & - \\
HPSv2~\citep{hpsv2}          & 54.7 & - & - \\
PickScore~\citep{kirstain2023pick}      & 58.6 & - & - \\
\midrule
\multicolumn{4}{c}{Qwen2.5-VL-7B-based evaluators} \\
\midrule
Qwen2.5-VL-7B~\citep{qwen25vl} & 50.4 & 57.8 & 53.7 \\
VQAScore~\citep{lin2024evaluating}    & 58.3 & - & - \\
HPSv3~\citep{ma2025hpsv3}          & 60.2 & - & - \\
EditReward~\citep{wu2025editreward}    & - & 67.2 & - \\
% LlavaCritic~\citep{xiong2025llava}    & - & - & 48.5 \\
UnifiedReward~\citep{wang2025unifiedreward}  & 59.8 & - & 55.1  \\
\bottomrule[1.2pt]

\end{tabular}


}
\caption{Other evaluators' accuracies on MMRB2. *For editing we use the single-image subset; for reasoning we use the text-only-output subset, ensuring fair comparison among evaluators.}
\label{tab:mllm_results_task}
\end{minipage}
\end{table*}




==> tables/pointwise_pairwise.tex <==
\begin{table}[ht]
\centering
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{ccccc}
\toprule[1.2pt]
Task & Judge & Type & Acc & 
\begin{tabular}[c]{@{}c@{}}Consist.\\Acc\end{tabular} \\
\midrule[1.2pt]
Image Gen & UnifiedReward & Point \\
Image Gen & UnifiedReward & Pair \\
\midrule
Image Edit &EditReward & Point \\
Image Edit &EditReward & Pair \\
\midrule
Reasoning & UnifiedReward & Point \\
Reasoning & UnifiedReward & Pair \\
\bottomrule[1.2pt]
\end{tabular}
}
\caption{Pointwise v.s. Pairwise}
\label{tab:Pointwise_vs_Pairwise}
\end{table}

==> tables/task_specific_evaluators.tex <==
% \begin{table}[ht]
% \centering
% \resizebox{0.3\textwidth}{!}{%
% \begin{tabular}{lccc}
% \hline
% Judge & 
% \begin{tabular}[c]{@{}c@{}}Image\\Gen\end{tabular} & 
% \begin{tabular}[c]{@{}c@{}}Image\\Edit\end{tabular} & 
% \begin{tabular}[c]{@{}c@{}}Visual\\Reasoning\end{tabular} \\
% \hline\hline
% \multicolumn{4}{l}{\textbf{MLLM-as-a-judge}} \\
% Qwen 2.5 7B &  &  &  \\
% GPT-4o &  &  &  \\
% GPT 5 &  &  &  \\
% \hline
% \multicolumn{4}{l}{\textbf{Other metrics}} \\
% CLIPScore &  & - & - \\
% VQAScore &  & - & - \\
% \hline
% \multicolumn{4}{l}{\textbf{Rewards trained with human preferences}} \\
% ImageReward &  &  &  \\
% HPSv2 &  &  &  \\
% PickScore & & & \\
% EditReward & & & \\
% LlavaCritic & - & -  &  \\
% UnifiedReward &  &  & 55.1  \\
% \hline
% \end{tabular}
% }
% \caption{Task specific evaluator performance. Image editing only contain single-image editing. Reasoning only contains single image + text.}
% \label{tab:mllm_results}
% \end{table}

==> tables/unused_app_tab567.tex <==
\begin{table}[]
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccc}
\hline
Judge & 
\begin{tabular}[c]{@{}c@{}}\shortmmrb:\\ Image\\ Generation\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\shortmmrb:\\ Image\\ Editing\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\shortmmrb:\\ Interleaved\\ 
Generation\end{tabular} & \begin{tabular}[c]{@{}c@{}}\shortmmrb:\\ Multi-modal\\ Reasoning\end{tabular} \\ \hline \hline
Gemini 2.5 Pro & & & & \\
Gemini 2.5 Flash & & & & \\
GPT 5 & & & & \\
GPT 4.1 & & & & \\
GPT 4o & & & & \\
Gemma 3 27B & & & & \\
Gemma 3 12B & & & & \\
Gemma 3 4B & & & & \\
Qwen 2.5 72B & & & & \\
Qwen 2.5 7B & & & & \\
Llama 3.2 11B & & & & \\
LLaVa-Critic~\citep{xiong2025llava} & & & & \\
UnifiedReward-Und~\citep{wang2025unified} & & & & \\
\hline
\end{tabular}
}%
\caption{Agreement rates (\%) between judges and human annotators on \longmmrb. Higher values indicate better alignment with human preferences.}
\label{tab:mllm_results}
\end{table}


% ==========================================
% Table 3: Detailed Judge Performance Breakdown
% ==========================================

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccc}
\toprule
\textbf{Task} & \textbf{Judge} & \textbf{Overall (\%)} & \textbf{Same-Model (\%)} & \textbf{Different-Model (\%)} \\
\midrule
\midrule
\midrule
\bottomrule
\end{tabular}
}%
\caption{Detailed performance breakdown of top 5 judges per task showing overall agreement, same-model pairs, and different-model pairs with human preferences.}
\label{tab:judge_detailed}
\end{table}


% Table 2: Model Performance by Rank
\begin{table}[h!]
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{4pt}
\small
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{L{1cm} L{2.5cm} L{4cm} L{3cm}}
\toprule
\textbf{Rank} & \textbf{Task} & \textbf{Model} & \textbf{Win Rate (\%)} \\
\midrule
\bottomrule
\end{tabular}
}%
\caption{Model win rates (\%) on \longmmrb~ranked by performance within each task. Win rate is computed as (wins + 0.5 × ties) / total comparisons.}
\label{tab:model_performance}
\end{table}
